ESPPU INPUT: C$^3$ within the "Linear Collider Vision"

The Linear Collider Vision calls for a Linear Collider Facility with a physics reach from a Higgs Factory to the TeV-scale with $e^+e^{-}$ collisions. One of the technologies under consideration for the accelerator is a cold-copper distributed-coupling linac capable of achieving high gradient. This technology is being pursued by the C$^3$ collaboration to understand its applicability to future colliders and broader scientific applications. In this input we share the baseline parameters for a C$^3$ Higgs-factory and the energy reach of up to 3 TeV in the 33 km tunnel foreseen under the Linear Collider Vision. Recent results, near-term plans and future R\&D needs are highlighted.

==> authors.tex <==
\begin{tcolorbox}[title=NOTES TO CONTRIBUTORS. PLEASE READ BEFORE EDITING]
\textbf{Deadlines:}
\begin{itemize}
    \item 31st January 2024 - Midnight EST:
        \begin{itemize}
            \item Final draft to circualte with LC vision.
        \end{itemize}
\end{itemize} 

Each file has a \textit{compile.tex} file.
Compiling this file will show only your chapter.
This prevents long wait times for compiling the whole document.
For the same reason, please only upload figures which are a reasonable filesize (e.g. kB rather than MB).
Otherwise large figures will be compressed.\\

Adding extra packages?
Please define it in \textit{packages.tex}, not in \textit{main.tex}.\\

Sections are to be labelled  \textbackslash label\{1:secname:sec\}, where the number indicates Part 0, 1 or 2, and \textit{secname} = 'intro', 'front', 'highacc' etc.
Subsections are to be labelled as \textbackslash label\{1:secname:sec:subsecname\}.
Figures as \textbackslash label\{1:secname:fig:figname\}. 
Tables as \textbackslash label\{1:secname:tab:tabname\}.\\

If you are including parameter tables, please also update the parameter spreadsheet.

Please use siunitx package as much as possible when defining units, for consistency. 
E.g. {\SI{10}{\tera\electronvolt}, \si{\tesla\per\meter\squared}, \num{2.99E8}} \\

The journal has requested for one bibliography for the whole report.
Please include in BibTeX style in \textit{bib/bibliography.bib}.\\

(Style preference) Please write one sentence per LaTeX line, for readability. \\

Any further comments or questions on style or formatting, please contact \textit{nanni@slac.stanford.edu}.
 \end{tcolorbox}


 \clearpage

==> titlepage.tex <==

%\small{Where we are now}}
\begin{picture}(0.001,0.001)
\put(-10,-30){\includegraphics[width=3.3cm]{FiguresFrontMatter/C3.png}}
\centering
\put(-10,-50){\Huge \bfseries		
\CCC within the "Linear Collider Vision"}
\put(-10,-60){\huge \bfseries		
Input for the European Strategy for Particle Physics}

%\put(65,-250){\includegraphics{FiguresFrontMatter/LogoOutline-Black-02.png}}

%\keywords{Collider, Higgs Factory, accelerator physics, technology}

\end{picture}
